CSI-Net: Unified Human Body Characterization and Pose Recognition

We build CSI-Net, a unified Deep Neural Network~(DNN), to learn the representation of WiFi signals. Using CSI-Net, we jointly solved two body characterization problems: biometrics estimation (including body fat, muscle, water, and bone rates) and person recognition. We also demonstrated the application of CSI-Net on two distinctive pose recognition tasks: the hand sign recognition (fine-scaled action of the hand) and falling detection (coarse-scaled motion of the body).

==> tex/1todo.tex <==
\section{To Do: May 15, 2018}

\begin{enumerate}

\item to visualize and explain encoded maps


% \item to revise related work(before 4.25)
% \item \blue{to complete experimental detail(before 4.24)}
% \item \blue{tomorrow, to look back signal model description(4.23-4.25)}

% \item \blue{to complete basic results of experiments(before 4.29)}
% \item to visualize and explain networks(4.23-5.5) 
% \item \blue{to revise abstract and introduction(before 5.3)}
% % \item revising twice and twice before submission
% \item to revise discussion (before 5.3)
% % \item to complete conclusion(before 5.5)

% \item biometrics prediction? or physiological index prediction?  measurement or something else
% \item CSI variance? CSI variation? or CSI time series/sequence?
% \item handcrafted features, manually determined features?
% \item fall, fallen or falling detection?



\end{enumerate}


==> tex/appnet.tex <==
% 作者：Fantasy
% 链接：https://www.zhihu.com/question/29803796/answer/137098435
% 来源：知乎
% 著作权归作者所有。商业转载请联系作者获得授权，非商业转载请注明出处。


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% shared layers 

\begin{table}
\centering
% \begin{minipage}{0.8\linewidth}

\begin{tabular}{|l|l|l|}

                                                                                   
\hline

layer name         &  \multicolumn{1}{c|}{layer parameters  }                                                                        & output size        \\ \hline
 transposedconv\_1           &  \multicolumn{1}{c|}{$4\times4$,384,stride=2,padding=1 }                                                                                     & $384\times2\times2$                 \\ \hline
 
  transposedconv\_2           &  \multicolumn{1}{c|}{$4\times4$,192,stride=2,padding=1 }                                                                                     & $192\times4\times4$                 \\ \hline
 
 transposedconv\_3           &  \multicolumn{1}{c|}{$3\times3$,96,stride=2,padding=1  }                                                                                    & $96\times7\times7$                 \\ \hline 
 
 transposedconv\_4           &  \multicolumn{1}{c|}{$4\times4$,48,stride=2,padding=1 }                                                                                     & $48\times14\times14$                 \\ \hline

 transposedconv\_5           &  \multicolumn{1}{c|}{$4\times4$,24,stride=2,padding=1  }                                                                                    & $24\times28\times28$                 \\ \hline

 transposedconv\_6          &  \multicolumn{1}{c|}{$4\times4$,12,stride=2,padding=1 }                                                                                     & $12\times56\times56$                 \\ \hline
 
  transposedconv\_7           & \multicolumn{1}{c|} {$4\times4$,6,stride=2,padding=1      }                                                                                & $6\times112\times112$                 \\ \hline
  
   transposedconv\_8           & \multicolumn{1}{c|}{ $4\times4$,6,stride=2,padding=1     }                                                                                 & $6\times224\times224$                 \\ \hline
   
    conv1           & \multicolumn{1}{c|}{$7\times7$,64,stride=2,padding=3 }                                                                                    & $64\times112\times112$                 \\ \hline
    
       max\_pool           & \multicolumn{1}{c|}{$3\times3$, stride=2,padding=1 }                                                                                    & $64\times56\times56$                 \\ \hline
    
    % conv2_x
\multirow{3}{*}{conv2\_x} & \multicolumn{1}{c|}{\multirow{3}{*} {$\begin{bmatrix}3\times3, & 64\\ 3\times3, & 64\end{bmatrix}\times 2$}} & \multirow{3}{*}{$64\times56\times56$} \\ 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\\hline



    % conv3_x
\multirow{3}{*}{conv3\_x} & \multicolumn{1}{c|}{\multirow{3}{*} {$\begin{bmatrix}3\times3, & 128\\ 3\times3, & 128\end{bmatrix}\times 2$}} & \multirow{3}{*}{$128\times28\times28$} \\ 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\\hline


    % conv4_x
\multirow{3}{*}{conv4\_x} & \multicolumn{1}{c|}{\multirow{3}{*} {$\begin{bmatrix}3\times3, & 256\\ 3\times3, & 256\end{bmatrix}\times 2$}} & \multirow{3}{*}{$256\times14\times14$} \\ 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\\hline

    % conv5_x
\multirow{3}{*}{conv5\_x} & \multicolumn{1}{c|}{\multirow{3}{*} {$\begin{bmatrix}3\times3, & 512\\ 3\times3, & 512\end{bmatrix}\times 2$}} & \multirow{3}{*}{$512\times7\times7$} \\ 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} \\\hline

\end{tabular}
\caption{Shared layers of all tasks. These layers consist of generation stage from layer of transposedconv\_1 to layer of transposedconv\_8 and part of feature learning stage from layer conv1 to layer of conv5\_x. The layers of generation stage generate data with size of $6\times224\times224$. The following feature learning layers are part of ResNet-18\cite{he2016deep} and produce data with size of $512\times7\times7$, which later is fed to the branch that belongs to each specific task.}

\label{tab:shared}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% table for biometrics estimation
\begin{table}[h]

\centering
\begin{tabular}{|l|l|l|}
\hline

layer name         &  \multicolumn{1}{c|}{layer parameters  }                                                                        & output size        \\ \hline
conv\_6           &  \multicolumn{1}{c|}{$3\times3$,512,stride=2,padding=1 }                                                                                     & $512\times4\times4$                 \\ \hline
 
conv\_7           &  \multicolumn{1}{c|}{$4\times4$,256,stride=2,padding=1 }                                                                                     & $256\times2\times2$                 \\ \hline

       ave\_pool           & \multicolumn{1}{c|}{$2\times2$, padding=0 }                                                                                    & $256$                 \\ \hline
       
             fc           & \multicolumn{1}{c|}{4-d fc, relu, L1 }                                                                                    & $4$                 \\ \hline
       
\end{tabular}
\caption{Biometrics estimation branch. This branch is paralleled with Person Recognition Branch showed in \Table{humanbranch}, and follows at the end of conv5\_x in \Table{shared}. This branch is composed of 2 \textit{convolution} layers, 1 \textit{average pool} layer and 1 fully-connected layer. Because we are to estimate 4 biometrics, we set the dimension of output 4.}
\label{tab:biobranch}
\end{table}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% table for human identification
\begin{table}[h]

% \begin{minipage}{0.8\linewidth} 
\centering
\begin{tabular}{|l|l|l|}
\hline

layer name         &  \multicolumn{1}{c|}{layer parameters  }                                                                        & output size        \\ \hline
conv\_6           &  \multicolumn{1}{c|}{$3\times3$,512,stride=2,padding=1 }                                                                                     & $512\times4\times4$                 \\ \hline
 
conv\_7           &  \multicolumn{1}{c|}{$4\times4$,256,stride=2,padding=1 }                                                                                     & $256\times2\times2$                 \\ \hline

       ave\_pool           & \multicolumn{1}{c|}{$2\times2$, padding=0 }                                                                                    & $256$                 \\ \hline
       
             fc           & \multicolumn{1}{c|}{30-d fc, softmax, cross entropy }                                                                                    & $30$                 \\ \hline
       
\end{tabular}
% \end{minipage}
\caption{Person recognition branch. This branch parallels with biometrics estimation branch showed in \Table{biobranch}, and follows at the end of conv5\_x in \Table{shared}. This branch is composed of 2 \textit{convolution} layer, 1 \textit{average pool} and 1 \textit{fully-connected} layer. Because we are to identify 30 subjects, we set the dimension of output 30.
}

\label{tab:humanbranch}
\end{table}






\begin{table}[h]

% \begin{minipage}{0.8\linewidth} 

\centering
\begin{tabular}{|l|l|l|}
\hline

layer name         &  \multicolumn{1}{c|}{layer parameters  }                                                                        & output size        \\ \hline
conv\_6           &  \multicolumn{1}{c|}{$3\times3$,256,stride=2,padding=1 }                                                                                     & $256\times4\times4$                 \\ \hline
 
conv\_7           &  \multicolumn{1}{c|}{$4\times4$ 128,stride=2,padding=1 }                                                                                     & $128\times2\times2$                 \\ \hline

       ave\_pool           & \multicolumn{1}{c|}{$2\times2$, padding=0 }                                                                                    & $128$                 \\ \hline
                    fc           & \multicolumn{1}{c|}{10-d fc, softmax, cross entropy }                                                                                    & $10$                 \\ \hline
       
\end{tabular}
\caption{Sign recognition branch. The shared layers showed in \Table{shared} and layers in this branch form a \net that used for recognizing human finger sign. This branch consists of 2 \textit{convolution} layer, 1 \textit{average pool} and 1 \textit{fully-connected} layer. Because we are to recognize 10 hand signs (from number 0 to number 9),  we set the dimension of output 10. Comparing to the branch for biometrics estimation and person recognition, we reducing the output size of each layer for avoiding overfitting is because we consider the complexity of this task is lower than the above. }\label{tab:signbranch}

\end{table}
% \end{minipage}



% \begin{minipage}{0.8\linewidth} 

\begin{table}[h]
\centering
\begin{tabular}{|l|l|l|}
\hline

layer name         &  \multicolumn{1}{c|}{layer parameters  }                                                                        & output size        \\ \hline
conv\_6           &  \multicolumn{1}{c|}{$3\times3$,256,stride=2,padding=1 }                                                                                     & $256\times4\times4$                 \\ \hline
 
conv\_7           &  \multicolumn{1}{c|}{$4\times4$,128,stride=2,padding=1 }                                                                                     & $128\times2\times2$                 \\ \hline

       ave\_pool           & \multicolumn{1}{c|}{$2\times2$, padding=0 }                                                                                    & $128$                 \\ \hline
       
             fc           & \multicolumn{1}{c|}{2-d fc, softmax, cross entropy }                                                                                    & $2$                 \\ \hline
       
\end{tabular}
\caption{Falling detection branch. The shared layers showed in \Table{shared} and layers in this branch form a \net that used for detecting human falling. This branch consists of 2 \textit{convolution layer}, 1 \textit{average pool} and 1 \textit{fully-connected} layer. Because we are to detect a human falling or not, we set the dimension of output 2. Comparing to the branch for biometrics estimation and person recognition, we reducing the output size of each layer for avoiding overfitting is because we consider the complexity of this task is lower than the above. }\label{tab:fallbranch}
\end{table}


==> tex/body_model.tex <==
\section{Wireless Signal Model}\label{sec:model}

\begin{figure*}[t]
\includegraphics[width=.9\linewidth]{figs/body_model.pdf}
   \centering
\caption{Wireless signals model at the presence of human body. \textbf{Left:} A cross-slice image of a female body\cite{ackerman2000imaging}, where circled layers are the skin, fat, muscle, viscus and bone. \red{(we gray it to protect readers.)}~\textbf{Right:} We simplify human body as a cylinder of three layers with different dielectric properties\cite{gabriel1996dielectric}. The transmitting signals from the Transmitter interact with human body along multiple propagation paths before reaching the Receiver. Here we sketched two paths of the signals.}
\label{fig:body}
\end{figure*}

\sout{
To understand why human bodies, even without motion, introduces CSI variances, we propose a simplified model that illustrates the interaction between the human body and WiFi signals, as shown in \Figure{body}. 
%It also states the reason why WiFi has capability for our four human sensing tasks. 
%
Human body is a propagation medium of WiFi signals, and hence capable of effecting transmitted WiFi signals and introducing CSI variances. Its influence mainly includes the reflection, refringence, and absorption on WiFi signals. 
The left figure in \Figure{body} is a cross-slice image of a female body 
\cite{ackerman2000imaging}, where the tissue in the middle is the torso and two smaller ones are arms. The torso consists of several layers, such as skin, fat, muscle, viscus and bone, each of which has different dielectric properties\cite{gabriel1996dielectric}. The signals from the transmitter reflects and refracts when propagating through theses layers along multiple propagation paths before reaching the receiver. 
For easy illustration,  
% Inspired by this work, 
we simplify the human body as a cylinder of three layers with different dielectric properties, and sketch two propagation paths of WiFi signals (as plotted in the right subfigure of \Figure{body}) at the presence of human body. Note that we ignore the influence from other objects in the environment for focusing on human body.}%without loss of generality. 
% \textbf{what the three layers are???} 
%reduce the complexity of human body is because that human body is an irregular geometrical object and hardly modeled. 



% human body is an irregular geometrical object and hardly modeled, 
% we reduce its complexity inspired by the left figure of \Figure{body}, %which is
% a cross slice image of a female\cite{ackerman2000imaging}, where two small circles are the arms and the big one is the torso. We focus on the torso and find out that the human body consists of several layers of tissue such as skin, fat and muscle, so we sketch a human body with three layer at the right that illustrating the propagation routes of the WiFi wave in the human body. 

\sout{Existing work\cite{gabriel1996dielectric} has experimentally confirmed that the presence of human body effects certain spectrum of wireless waves, including WiFi. 
%  \red{Delete This is mainly because the dielectric properties of human body is different from that of the furniture, wall and floor.}
\Table{tissue} shows dielectric properties of different tissues, such as permittivity and conductivity, around the central frequency of WiFi, i.e., 2.4GHz and 5GHz, at the temperature of $37.0 ^{\circ}C$/$98.6 ^{\circ}F$\cite{gabriel1996dielectric}. 
}

\begin{table}[t]
\centering
\begin{tabular}{l|l|l|l}
\hline
\textbf{Tissues}                           & \textbf{Frequency} & \textbf{Permittivity} & \textbf{Conductivity (S/m)} \\ \hline
\multirow{2}{*}{Skin (Dry)}                & 2.4GHz             & 39.81                 & 1.78                        \\ \cline{2-4} 
                                           & 5GHz               & 33.11                 & 3.98                        \\ \hline
\multirow{2}{*}{Skin (Wet)}                & 2.4GHz             & 39.81                 & 2.24                        \\ \cline{2-4} 
                                           & 5GHz               & 35.48                 & 5.62                        \\ \hline
\multirow{2}{*}{Fat (Average Infiltrated)} & 2.4GHz             & 10.23                 & 0.32                        \\ \cline{2-4} 
                                           & 5GHz               & 8.91                  & 0.71                        \\ \hline
\multirow{2}{*}{Fat (Not Infiltrated)}     & 2.4GHz             & 5.62                  & 0.1                         \\ \cline{2-4} 
                                           & 5GHz               & 5.59                  & 0.32                        \\ \hline
\multirow{2}{*}{Muscle}                    & 2.4GHz             & 50.12                 & 2.51                        \\ \cline{2-4} 
                                           & 5GHz               & 44.67                 & 5.62                        \\ \hline
\multirow{2}{*}{Bone (Cortical)}           & 2.4GHZ             & 11.22                 & 0.56                        \\ \cline{2-4} 
                                           & 5GHz               & 8.91                  & 1.12                        \\ \hline
\multirow{2}{*}{Bone (Cancellous)}         & 2.4GHz             & 15.85                 & 0.71                        \\ \cline{2-4} 
                                           & 5GHz               & 14.13                 & 1.41                        \\ \hline
\end{tabular}

\caption{Dielectric characteristics, permittivity and conductivity of human tissues at 2.4GHz and 5GHz WiFi band. These tissues have different dielectric characteristics in each band, which generate CSI variances in the received WiFi signals.}

\label{tab:tissue}
\end{table}

With above observation, we analyze in depth how the amplitude, frequency and phase of the WiFi signals vary at the presence of the human body. Formally, WiFi signals is denoted as $x = Asin(\omega t + \phi)$,
where $A$, $\omega$ and $\phi$ are the amplitude, frequency and initial phase, respectively. We denote the WiFi signals emitted from the transmitter as $X$. Suppose that the human body influence the signal according to a function $f(\cdot)$. At the receiver, the WiFi signals thereby become $f(X)$. %\blue{The following stands for signal variation along single propagation path.}

\textbf{Amplitude:} The amplitude is a measure of the signal power. The power of signals decays when propagating in a medium due to absorption effect of the medium. As aforementioned, human body can be considered as a medium with different tissue layers. 
The electromagnetic wave transmission theories, Friss Transmission Equation\cite{shaw2013radiometry} and Beer-Lambert Law\cite{mayerhofer2016employing}, can be used to compute the amplitude decay.

\textbf{Frequency:} According to Doppler Effect\cite{chen2006micro}, the frequency of the WiFi signals vary when a human moves. The variation of frequency is
\begin{equation}
 \Delta  \omega = \frac{ \pm v_o}{v} \omega
\end{equation}
where $v$ is the speed of WiFi signals in a given medium, $v_o$ is the moving speed of the person. For example, if $v_o=1m/s$, the frequency variation $\Delta w$ approximates 17Hz at the central frequency of 5GHz. 

\textbf{Phase:} The phase variation, $\Delta \Phi$ ,is as follows,
\begin{equation}
\Delta \Phi  = mod(2\pi \frac{d}{\lambda} , 2\pi) 
\end{equation}
where $mod(\cdot)$ is a modulo operator, $d$ is the length of wave propagation in a layer, and $\lambda$ is the wavelength of WiFi signals at this tissue layer. $d$ and $\lambda$ are highly related to the body shape and electromagnetic properties of the certain human body.  

In practice, WiFi signals interact with the human body along multiple propagation paths. As illustrated in \Figure{body}, the multi-path propagation makes it extremely challenging to parse the aforementioned CSI variances in amplitude, frequency and phase. To address this challenge, we resort to the nonlinear mapping ability of deep learning to analyze the joint CSI variances of multi-path propagations.
%
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


==> tex/discussion.tex <==
\section{Limitation and Future Work}\label{sec:discussion}





For the task of activity recognition, current version of CSI-Net requires subjects to act the predefined postures then makes prediction among these postures. This requirement is acceptable for activity-specific systems such as those detect the elderly falling. 
However, there still exist situations that require human motion to be recognized continuously like the surveillance system. Our future work focuses on addressing this limitation.

Recalling that current CSI-Net generates spatially-encoded maps and process CSI data as images. To perform continuous human motion recognition, CSI-Net should \textbf{learn spatiotemporal-encoded maps} from CSI sequences. In this way, CSI sequences can be treated as videos. Consulting techniques in computer vision for videos, we are considering two methods to extend CSI-Net for continuous human motion recognition.

\begin{enumerate}
\item \textbf{Spatio-temporal Convolution Operation:} 
Three-Dimensional Convolution (C3D)\cite{tran2015learning}, Convolution-Deconvolution-Convolution (CDC)\cite{shou2017cdc} and Temporal Preservation Convolution (TPC)\cite{yang2018exploring} were proposed to conduct
%conduce 
action recognition from videos. Those approaches not only extract semantic information (spatially-encoded) of individual video frames but also learn temporal information from continuous video clips. Their experimental results outperform some work built on RNNs like LSTM\cite{donahue2015long,yeung2018every}. CSI-Net is based on single-image convolution, so it could be easily extended with spatio-temporal convolution operations for continuous human motion recognition.  

\item \textbf{Large Dataset plus Very Deep 3D CNNs:} 
Another way is to devote to a large dataset and apply common 3D filters to optimize very deep CNNs like ResNet-152\cite{he2016deep}. This technology road-map was verified in \cite{hara2017can} that utilizes Kinetics dataset\cite{kay2017kinetics} (300K videos) and very deep 3D CNNs for action recognition, such as ResNet-200\cite{he2016deep}, DenseNet-201\cite{huang2017densely} and ResNeXt-101\cite{xie2017aggregated}. Following this road-map, we are considering to build a large dataset. However, comparing to computer vision tasks, 
%situation is much tougher in 
% \blue{
WiFi-based human sensing is more complicated because CSI is highly correlated with Tx/Rx deployed surroundings. This correlation would undermine the CSI-Net even being optimized by a very large dataset, once it was to test in a new environment. Thus, de-correlating the CSI with environments is also a significant future work when building large datasets.     
 
\end{enumerate}





% In the techniques of computer vision for videos, three-dimensional convolution kernels (3D) are 


% 3D convolution kernel 

% Some algorithms, such as C3D\cite{tran2015learning}, CDC\cite{shou2017cdc}, and TPC\cite{yang2018exploring} are proposed to solve a similar problem in the computer vision domain, where human activities can be recognized with several successive frames in a video stream. We can apply these algorithms at the beginning of the feature learning stage in CSI-net, which will make CSI-net practical for human activity recognition.  



% CSI-net may annoy people if asking them to repeat activities many times for obtaining enough training instances. To reduce the number of repeating activities, we can develop an algorithm that does not require the whole corresponding CSI sequence but a small part of it. 

% Although, the experimental results demonstrate the ability and generality of CSI-net in inspecting and monitoring human state, CSI-Net still has some limitations. In this section, we discuss its limitations and propose potential solutions.
% \textbf{don't understand this point!!!}

% \begin{enumerate}
% \item CSI-net lacks competitiveness comparing with MUSIC-based approaches in indoor localization because of an inescapable work of CSI collection and a lower accuracy, which is a systematic weakness. However, CSI-net may has potential advantages in clustering crowds, which is tough for MUSIC-based approaches.

% \item
% CSI-net may annoy people if asking them to repeat activities many times for obtaining enough training instances. To reduce the number of repeating activities, we can develop an algorithm that does not require the whole corresponding CSI sequence but a small part of it. 
% %Thus, the whole CSI sequence can be split to much more training instances. So that, 
% The problem comes to how to recognize an activity using a number of parts of CSI sequence. Some algorithms, such as C3D\cite{tran2015learning}, CDC\cite{shou2017cdc}, and TPC\cite{yang2018exploring} are proposed to solve a similar problem in the computer vision domain, where human activities can be recognized with several successive frames in a video stream. We can apply these algorithms at the beginning of the feature learning stage in CSI-net, which will make CSI-net practical for human activity recognition.  

% \end{enumerate}



==> tex/layer_model.tex <==
\section{Layered Tissue Model}\label{sec:model}%\marginpar{Review 4, show WiFi signals reflecting from one human can contain so much fine grained information about human body. Review 5, explanation of WiFi signal variation in relation with presence of human body.}

\begin{figure*}[t]
\includegraphics[width=.9\linewidth]{figs/body_model.pdf}
   \centering
\caption{Wireless signals model at the presence of human body. \textbf{Left:} A cross-slice image of a female body\cite{ackerman2000imaging}, where circled layers are the skin, fat, muscle, viscus and bone. (we gray it to protect readers.)~\textbf{Right:} We simplify human body as a cylinder of three layers with different dielectric properties\cite{gabriel1996dielectric}. The transmitting signals from the Transmitter interact with human body along multiple propagation paths before reaching the Receiver. Here we sketched two paths of the signals.}
\label{fig:body}
\end{figure*}


\begin{table}[t]
\centering
\begin{tabular}{l|l|l|l}
\hline
\textbf{Tissues}                           & \textbf{Frequency} & \textbf{Permittivity} & \textbf{Conductivity (S/m)} \\ \hline
\multirow{2}{*}{Skin (Dry)}                & 2.4GHz             & 39.81                 & 1.78                        \\ \cline{2-4} 
                                           & 5GHz               & 33.11                 & 3.98                        \\ \hline
\multirow{2}{*}{Skin (Wet)}                & 2.4GHz             & 39.81                 & 2.24                        \\ \cline{2-4} 
                                           & 5GHz               & 35.48                 & 5.62                        \\ \hline
\multirow{2}{*}{Fat (Average Infiltrated)} & 2.4GHz             & 10.23                 & 0.32                        \\ \cline{2-4} 
                                           & 5GHz               & 8.91                  & 0.71                        \\ \hline
\multirow{2}{*}{Fat (Not Infiltrated)}     & 2.4GHz             & 5.62                  & 0.1                         \\ \cline{2-4} 
                                           & 5GHz               & 5.59                  & 0.32                        \\ \hline
\multirow{2}{*}{Muscle}                    & 2.4GHz             & 50.12                 & 2.51                        \\ \cline{2-4} 
                                           & 5GHz               & 44.67                 & 5.62                        \\ \hline
\multirow{2}{*}{Bone (Cortical)}           & 2.4GHZ             & 11.22                 & 0.56                        \\ \cline{2-4} 
                                           & 5GHz               & 8.91                  & 1.12                        \\ \hline
\multirow{2}{*}{Bone (Cancellous)}         & 2.4GHz             & 15.85                 & 0.71                        \\ \cline{2-4} 
                                           & 5GHz               & 14.13                 & 1.41                        \\ \hline
\end{tabular}

\caption{Dielectric characteristics, permittivity and conductivity of human tissues at 2.4GHz and 5GHz WiFi band. These tissues have different dielectric characteristics in each band, which generate CSI variances in the received WiFi signals.}

\label{tab:tissue}
\end{table}


Based on the layered tissue model in bio-eletromagnetics, we further explain how the human body, even without motions, can cause CSI variances and these variances are embedded with fine-grained human body information. 

In \Figure{body}~(left), we show a cross-slice image of a female body \cite{ackerman2000imaging}, where the bigger part in the middle is the torso, and two smaller parts are the arms.
Looking closely in the torso part, we can see several layers of human body, such as skin, the fat under skin, muscle, the fat on the viscera, viscera, bone, \etc. In \cite{gabriel1996dielectric}, dielectric characteristics of many body tissues have been measured at the regular body temperature ($37.0^{\circ}C$/$98.6 ^{\circ}F$). The results are selectively listed in \Table{tissue} at the EM frequency of 2.4GHz and 5GHz, \ie, frequencies in the WiFi bands. In \cite{christ2006characterization, christ2006dependence}, a human torso is considered as layered tissues with different dielectric parameters for studying the specific absorption rate on certain EM wave.

According to these works, for simplicity we sketch the layered tissue model in the context of WiFi communication systems in \Figure{body}~(right), in which the human body consists of 3 layers with different thickness and dielectric properties. In the figure, human body is considered as a propagation medium of WiFi signals, and hence capable of affecting transmitted WiFi signals and producing WiFi variances. Before reaching the receiver, the signals from the transmitter may be reflected or refracted when propagating through body layers along multiple propagation paths. For easy illustration, we only draw two propagation paths of WiFi signals. Note that for simplicity, we ignore the influence from other objects in the environment.

% \marginpar{Review 4, explanation the motivation of giving  \Table{tissue} and \Figure{body}}

Taking the path \#1 (plotted in the \Figure{body}~(right)) as an example, if we know the characteristics of this path, including the properties of each layer and EM frequency, we could calculate the body-information-embedded power decay and time delay when WiFi signals reaching the receiver. Next, we show how the body information is embedded into the received WiFi signals according to \cite{dove2014analysis}.

Formally, denote the WiFi signal emitted from the transmitter as $x$. The EM wave function is written as $x = Ae^{-j2\pi ft + \phi}$, where $A$, $f$ and $\phi$ are the amplitude, frequency and initial phase, respectively. Before formulating the impacts of human body and the air on the bypassing WiFi signals, we define some notations in \Table{symbols}.  

Time delay: the sum of propagation time delay in all medium. For each medium, the time delay equals to $t_i = d_i / v_i$. where $v_i$ is the speed of WiFi signals in this propagation medium, and is computed as $v_i = 1/\sqrt{\mu_i \varepsilon_i}$ \cite{guru2004electromagnetic}. For path \#1, the overall time delay is

\begin{equation}
t = \sum_{i=1}^{n}{d_i \sqrt{\mu_i \varepsilon_i}} + d_0 \sqrt{\mu_i \varepsilon_i}
\label{eq:td}
\end{equation}
where $n$ is the number of tissue layers. 

Power decay:  the product of power decay in all medium (\Table{symbols}). The overall power decay is computed as
\begin{equation}
A' = A c_0 \prod_{i=1}^{n}{c_i}
\label{eq:pd}
\end{equation}
Please refer to \cite{dove2014analysis} for a more comprehensive expression, which utilizes Friis Transmission Equation\cite{shaw2013radiometry} and Beer-Lambert Law\cite{mayerhofer2016employing} to compute power decay. Combining \Equation{td} and \Equation{pd}, the received WiFi signals are 
\begin{equation}
y = \uwave{\prod_{i=1}^{n}{c_i}e^{-j2\pi f\sum_{i=1}^{n}{d_i \sqrt{\mu_i \varepsilon_i}}}}\cdot c_0e^{-j 2\pi f d_0 \sqrt{\mu_i \varepsilon_i}}\cdot x
\end{equation}
Note that we mark the WiFi variation caused by the presence of human body with a wave line. From the equation, we know that the dielectric characteristics of body tissues such as thickness, permeability, permittivity \etc, are embedded into the received WiFi signals.

The layered tissue model indicates a reason why WiFi signals vary in amplitude and phase when different persons appear in the environment, \ie, different person has different tissue properties. Suppose we have received WiFi signals~(donated by $h$) and we want to characterize body information~($I$), such as to estimate body fat rate. Thus, we need to learn a mapping function $I=f(h)$. It is challenging to solve this problem analytically, we seek for deep learning to learn a approximation function by inputing a large dataset. Next, we talk details in the network framework.




% Moreover, the commercially available devices such as commodity body composition scales, \eg, Mi\textregistered ~\cite{mibodysscale} use the impedance of human body on bypass electricity to analyze the fine-grained body information, such as the body fat/muscle/water/bone rate. Very similar to this principle, we believe the fine-grained body information embedded in WiFi signals could also be extracted. Different from the contact devices above, parsing body characteristics from WiFi signals requires powerful nonlinear mapping algorithms, \ie, CSI-Net.



\begin{table}[t]
	\centering
	\begin{tabular}{l||l}
		\hline
		Symbols & Meaning                     \\ \hline 
        		$d_0$  &  Distance of signals propagating through the air\\ \hline
                $d_i$  &  Distance of signals propagating through the $i^{\text{th.}}$ layer of human body  \\ \hline
          $c_{0}$      & Power decay in the air \\ \hline
          $c_i$      & Power decay in the $i^{\text{th.}}$ layer of human body \\ \hline 
          $\mu_0$  & Permeability of the air \\ \hline
          $\mu_i$  & Permeability of the $i^{\text{th.}}$ layer of human body \\ \hline
		$ \varepsilon_0$  &  Permittivity of the air \\ \hline
		$ \varepsilon_i$  &  Permittivity of the $i^{\text{th.}}$ layer of human body \\ \hline
	\end{tabular}
	\caption{List of the mathematical symbols.}
	\label{tab:symbols}
\end{table}




% With above observation, we analyze in depth how the amplitude, frequency and phase of the WiFi signals vary at the presence of the human body. Formally, WiFi signals is denoted as $x = Asin(\omega t + \phi)$, where $A$, $\omega$ and $\phi$ are the amplitude, frequency and initial phase, respectively. We denote the WiFi signals emitted from the transmitter as $X$. Suppose that the human body influence the signal according to a function $f(\cdot)$. At the receiver, the WiFi signals thereby become $f(X)$. %\blue{The following stands for signal variation along single propagation path.}

% \textbf{Amplitude:} The amplitude is a measure of the signal power. The power of signals decays when propagating in a medium due to absorption effect of the medium. As aforementioned, human body can be considered as a medium with different tissue layers. 
% The electromagnetic wave transmission theories, Friis Transmission Equation\cite{shaw2013radiometry} and Beer-Lambert Law\cite{mayerhofer2016employing}, can be used to compute the amplitude decay.

% \textbf{Frequency:} According to Doppler Effect\cite{chen2006micro}, the frequency of the WiFi signals vary when a human moves. The variation of frequency is
% \begin{equation}
%  \Delta  \omega = \frac{ \pm v_o}{v} \omega
% \end{equation}
% where $v$ is the speed of WiFi signals in a given medium, $v_o$ is the moving speed of the person. For example, if $v_o=1m/s$, the frequency variation $\Delta w$ approximates 17Hz at the central frequency of 5GHz. 

% \textbf{Phase:} The phase variation, $\Delta \Phi$ ,is as follows,
% \begin{equation}
% \Delta \Phi  = mod(2\pi \frac{d}{\lambda} , 2\pi) 
% \end{equation}
% where $mod(\cdot)$ is a modulo operator, $d$ is the length of wave propagation in a layer, and $\lambda$ is the wavelength of WiFi signals at this tissue layer. $d$ and $\lambda$ are highly related to the body shape and electromagnetic properties of the certain human body.  

% In practice, WiFi signals interact with the human body along multiple propagation paths. As illustrated in \Figure{body}, the multi-path propagation makes it extremely challenging to parse the aforementioned CSI variances in amplitude, frequency and phase. To address this challenge, we resort to the nonlinear mapping ability of deep learning to analyze the joint CSI variances of multi-path propagations.
%
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


==> tex/net_tables.tex <==

\begin{table}[]
\centering
\begin{tabular}{|l|l|c|r|r|r|}

\hline
layer name   & output size              &biometrics prediction                                       & \multicolumn{1}{c|}{human identification } & output size              & layer name   \\ \hline
transconv\_1 & $2\times 2 \times 384$    & \multicolumn{2}{c|}{$4\times 4$, 384, stride=2, padding=1}                                              & $2\times 2 \times 384$    & transconv\_1 \\ \hline
transconv\_2 & $4\times 4 \times 192$   & \multicolumn{2}{c|}{$4\times 4$, 192, stride=2, padding=1}                                              & $4\times 4 \times 192$   & transconv\_2 \\ \hline
transconv\_3 & $7\times 7 \times 96$   & \multicolumn{2}{c|}{$3\times 3$, 96, stride=2, padding=1}                                               & $7\times 7 \times 96$   & transconv\_3 \\ \hline
transconv\_4 & $14\times 14 \times 48$ & \multicolumn{2}{c|}{$4\times 4$, 48, stride=2, padding=1}                                               & $14\times 14 \times 48$ & transconv\_4 \\ \hline
transconv\_5 & $28\times 28 \times 24$  & \multicolumn{2}{c|}{$4\times 4$, 24, stride=2, padding=1}                                               & $28\times 28 \times 24$  & transconv\_5 \\ \hline
transconv\_6 & $56\times 56 \times 12$  & \multicolumn{2}{c|}{$4\times 4$, 12, stride=2, padding=1}                                               & $56\times 56 \times 12$  & transconv\_6 \\ \hline
transconv\_6 & $112\times 112 \times 6$ & \multicolumn{2}{c|}{$4\times 4$, 6, stride=2, padding=1}                                                & $112\times 112 \times 6$ & transconv\_6 \\ \hline
transconv\_7 & $224\times 224 \times 3$ & \multicolumn{2}{c|}{$4\times 4$, 3, stride=2, padding=1}                                                & $224\times 224 \times 3$ & transconv\_7 \\ \hline
conv1     & $112\times112 \times 64$ & \multicolumn{2}{c|}{$7\times 7$, 64, stride=2, padding=3}                                               & $112\times112 \times 64$ & conv1     \\ \hline
max\_pool     & $56 \times 56 \times 64$ & \multicolumn{2}{c|}{$3\times 3$, max pool}                                                     & $56 \times 56 \times 64$ & max\_pool     \\ \hline

 &                                           &                                                                                        &                     &                                           &                           \\ %\cline{6-6}
conv2\_x     & $56 \times 56 \times 64$ & \multicolumn{2}{c|}{$\begin{bmatrix}3\times3, & 64\\ 3\times3, & 64\end{bmatrix}\times 2$}              & $56 \times 56 \times 64$ & conv2\_x     \\
 &                                           &                                                                                        &                     &                                           &                           \\ \cline{6-6}

\hline

 &                                           &                                                                                        &                     &                                           &                           \\ %\cline{6-6}

conv3\_x     & $28\times 28\times 128 $ & \multicolumn{2}{c|}{$\begin{bmatrix}3\times3, & 128\\ 3\times3, & 128\end{bmatrix}\times 2$}            & $28\times 28\times 128 $ & conv3\_x    
\\ 
 &                                           &                                                                                        &                     &                                           &                           \\ \cline{6-6}
\hline

 &                                           &                                                                                        &                     &                                           &                           \\ %\cline{6-6}
conv4\_x     & $14\times 14 \times 256$ & \multicolumn{2}{c|}{$\begin{bmatrix}3\times3, & 256\\ 3\times3, & 256\end{bmatrix}\times 2$}            & $14\times 14 \times 256$ & conv4\_x     \\ 
 &                                           &                                                                                        &                     &                                           &                           \\ \cline{6-6}


\hline

 &                                           &                                                                                        &                     &                                           &                           \\ %\cline{6-6}
conv5\_x     & $7\times 7 \times 512$   & \multicolumn{2}{c|}{$\begin{bmatrix}3\times3, & 512\\ 3\times3, & 512\end{bmatrix}\times 2$}            & $7\times 7 \times 512$   & conv5\_x     \\ 

 &                                           &                                                                                        &                     &                                           &                           \\ \cline{6-6}


\hline
conv6\_1     & $4\times 4 \times 512$   & \multicolumn{1}{l|}{$3\times 3, 512$, stride=2} & $3\times 3, 512$, stride=2      & $4\times 4 \times 512$   & conv6\_2     \\ \hline
conv7\_1     & $2\times 2 \times 256$  & \multicolumn{1}{l|}{$3\times 3, 256$, stride=2} & $3\times 3, 256$, stride=2      & $2\times 2 \times 256$  & conv7\_2     \\ \hline
avg\_pool1\_1 & 256                      & \multicolumn{1}{l|}{$2\times 2$, avg pool}   & $2\times 2$, avg pool        & 256                      & avg\_pool1\_2 \\ \hline
fc1\_1        & 4                       & \multicolumn{1}{l|}{4-d fc, relu}                      & 30-d fc, softmax                               & 30                        & fc1\_2        \\ \hline

\multicolumn{6}{l}{}  \\ \hline 

layer name    & output size            & sign recognition          & falling detection         & output size            & layer name    \\ \hline
avg\_pool1\_1 & $1\times 1 \times 512$ &  $7 \times7$, avg pool &  $7 \times7$, avg pool & $1\times 1 \times 512$ & avg\_pool1\_2 \\ \hline
fc1\_1        & $10$                   & 10-d fc, softmax          & 2-d fc, softmax           & $2$                    & fc1\_2        \\ \hline

\end{tabular}

\caption{One CSI-Net architecture on the basis of ResNet-18\cite{he2016deep}.
% for the task of human identification and biometrics(body fat, muscle, water and bone rate) prediction. 
\textbf{Upper:}
Through 7 transposed convolution operations, the $1\times 1\times 30$ input is converted to $224\times 224 \times 3$, then feed into the convolution operation of standard ResNet-18\cite{he2016deep} and becomes $7 \times7 \times 512$. Layers from transconv\_1 to conv5\_x are shared with both tasks, which correspond to the Generation Stage and Feature Extraction Stage. Two paralleled conv6, conv7 avg\_pool1 and fc1 are stacked for each task. The max pool and average pool perform downsample with stride 2.
\textbf{Lower:} Using one average pool layer (avg\_pool1\_1) and one fully-connected layer (fc1\_1) to replace layers from conv6 to fc1 makes a CSI-Net for sign recognition. Similarly, using one average pool layer (avg\_pool1\_2) and one fully-connected layer (fc1\_2) to replace layers from conv6 to fc1 makes a CSI-Net for falling detection.
}

\label{tab:net}
\end{table}

==> tex/r1.tex <==
\subsection{Meta-review}\label{sec:meta}
\textbf{From reviewer 1} 

(1) More details, hopefully in terms of both theoretical and empirical, on the design choice of placing a generative network in the middle.
 


\blue{Response:} We add more theoretical analysis about designing a generative network in the \Sec{input} and \Sec{generation}. Empirically, we add \Sec{v15} and \Table{v15}, where we compare 3 different methods of reshaping $1\times 1$ input tensor to $224\times 224$.

Theoretically, the generative network is critical to produce rich features and highly nonlinear transformation for our tasks. 

The signal amplitude of each channel (subcarrier) is the integral reflection of all transmitting paths. The spatial information of the environment and subjects are deeply embedded in the signal. Transforming the 1-dimensional-30-channel CSI data to biometric measures and action categories requires rich feature representations and highly nonlinear transformation.  However, 
%the ability of 
standard CNNs require 2D inputs (images) for spatial convolution. The spatial convolution expands 2D inputs into high-order channel-specific features at the expense of losing spatial resolution.  Usually, the bigger the input sizes, the deeper CNNs can be constructed, leading to more powerful CNNs. This is the key mechanism of the Generative adversarial network (GAN) current prevalence in computer vision. In particular, in DC-GAN~\cite{radford2015unsupervised}, a generative network transforms 1D random variables to 2D images. Only from the generated 2D images, the Discriminator networks for classification and regression can be used to complete complex tasks such as recognizing objects and activities. Our work follows the success of GAN, and uses a generative network to produce spatial coding of CSI. From the 2D representation of CSI data, feature learning and task-specific networks (similar to those CNNs that have proven effective in computer vision) were constructed to produce biometric measures and action categories.   

Empirically, we conduct a new baseline experiment to validate the effect of the generative network. In the new baseline, the generative network is replaced by bilinear interpolation (BI).  The CSI input is interpolated to input size of the features learning stage. The rest of the network was kept the same. For all the tasks in this paper, CNN with BI performed worse than the CNN with generative network. This demonstrates that generative networks effectively learn to encode the spatial information of the CSI data.\\ 



(2) More rationales behind the choice of ResNet-18 whose original image classification performance was outperformed by other well-known models.

\blue{Response:} We rewrite \Sec{feature_learning}. In this section, we give more rationales behind the choice of ResNet-18. In addition, we add \Sec{ablation}, \Table{backbone} and \Table{modelsize}, which show the results of 9 different well-known models, such as ResNet-101, ResNet-152, Inception-V3/V4, \etc, on our tasks. The result shows that ResNet-18 has the best balance between task complexity and data complexity.\\

% Following the insights in \cite{canziani2016analysis}, we select ResNet because it is generally more powerful than AlexNet, and has less parameters than VGG-nets, Inception Net and DenseNet. For our current experiments, we prefer not to use heavy networks because we have relatively small dataset (40K CSI samples) compared to benchmark computer vision databases (COCO dataset with 330K images). Heavy networks are prone to overfit.\\

\blue{\textit{Please see our responses for other comments in \Sec{other}.}}\\





==> tex/r1_full.tex <==
\subsection{Other comments }\label{sec:other}
\textbf{From reviewer 1}

(1) Why the particular choice of 30 x 1 x 1 tensor size was chosen? Why the other dimensions like [30/4] x 2 x 2 or [30/9] x 3 x 3 are not considered? What differences are expected if one chooses a different dimension? Also, why the choice of 30 x 1 x 1 means no loss of generality?.

\blue{Response:} We use Linux 802.11n CSI tool and Intel 5300 NICs, \href{https://dhalperi.github.io/linux-80211n-csitool/}{https://dhalperi.github.io/linux-80211n-csitool/}, which report CSI of 30 different channels, \ie, 30 subcarriers with different frequencies. We take 30 as the input channels. Since CSI-Net is to detect human stationary gestures, we expect that even one sample can be used to represent a gesture. Thus, we reshape the $30\times 1$ to $30\times 1 \times 1$.

We do not consider other dimensions because of
%is to respect 
the properties of CSI. If we reshape CSI to [30/4]x2x2, then in a 2x2 matrix, every subcarrier has neighbors at its left/right and upside/downside directions. However, this spatial correlation does not exist among WiFi channels. Considering this, we did not choose the size of [30/4] x 2 x 2 and [30/9] x 3 x 3. 

We agree that this is an ambiguity in `loss of generality'. In \Table{csi_tool}, we show 3 CSI tools, which report CSI with different channel numbers. We used `loss of generality' is to take the Linux 802.11n CSI tool~(30 channels) for example. To avoid this ambiguity, we omit this phrase. \\



(2) Why the generation stage is required? What if the input layer size is chosen to be spatially larger, does it still require a generation stage? Is the purpose of the generation stage simply to make the input size compatible to an off-the-shelf model which takes an input of 224 x 224? If so, isn't there any simpler way to reshape the input, rather than going through extensive computation of multiple layers of deconvolution?

\blue{Response:} We think the generation stage could spatially convert the information embedded in channels. Please see \Sec{meta}~(From reviewer 1, (1)) for more explanation.
%to information embedded 
% This is a very significant operation for the input with height/width of $1 \times 1$. 
In the revised version, we detail why we apply the generation stage in \Sec{input} and \Sec{generation}.

\blue{Response:} If the input layer size is sufficiently large, \eg, 224x224, then yes, the generation stage is not necessary.  Generally, bigger input layer size allows deeper neural networks, which leads to more powerful feature learning capability.

As mentioned above, the generation stage can introduce nonlinear mapping ability into CSI-Net, potentially increasing the accuracy. To validate other reshaping methods, we use \textit{bilinear} interpolation to resize $1 \times 1$ tensor to $224 \times 224$ tensor, and find that it also works well. This inspired us to find a better way to reshape the input size to $224 \times 224$. Then we propose CSI-Net V1.5, which is lighter but works better than CSI-Net. We add \Sec{v15} to show this improvement. We sincerely thank you for this inspiration. \\




(3) Why such successive filters are essentially required, given that the eventual purpose is denoising. Wouldn't be a single Butterworth filter, or even a moving average sufficient?

\blue{Response:} In our work, we first use time domain filters to denoise. The \textit{median filter} is to remove extremely high/low values, and the \textit{mean filter} is to smooth the series. Then, the Butterworth filter is contentiously denoising in frequency domain. In this way, the denoising can take effect. 

We thank the valuable advice. It may be better if sufficiently testing possible filters. However, for the reason of applying Data Augmentation Algorithm, shown in \Sec{dataset}, we randomly shuffled the time series, which made it impossible for us to obtain another augmented dataset whose each item is augmented by the same samples as the current one. We will try your advice in our future work. In this paper, considering the filter operation is very fast if using Matlab function, we leave the filter design strategy unchanged.   \\ 

(4) How susceptible is the body composition of the same person depending on different activities the person has done? Such as after a workout, after eating, after hydration, after returning from a bathroom, etc.? In essence, is the intra-person body composition data robust enough to authenticate a person at a different time of day Similarly, are the inter-person body composition data discriminative enough to identify a person out of many? What is the reasonable number of people each of which could be identified among them based on their body composition data? 

\blue{Response:} These concerns are valuable and deserve extensive experiments. In this paper, we focused on building CSI-Net as a generic model for WiFi sensing tasks.  Our future work will include extensive data collection and experiment on subjects under different physical conditions.

% Actually, we are also devoted to make CSI-Net more practical and robust in real life. 
% Currently, we are collecting more data in different environment, time, even the presence of other persons. We are also modifying CSI-Net for new application. 
% (2) It is counterintuitive that other models that achieved higher records in the original image classification challenges (e.g., ResNet 152, Inception v4) are not chosen. 

==> tex/r3.tex <==
\noindent \textbf{From reviewer 3}

(1) Clarify the adaptation of DNN to CSI data

\blue{Response:}  
We give more explanation on applying DNN to CSI data in \Sec{input} and \Sec{generation}. 
Besides, we also add \Sec{prior_deep} to show some prior works that have applied SHADOW neural network on CSI data.


Our adaption of DNN to CSI data lies in two folds:

First, we construct input tensor such that 2D convolutions are performed within CSI channels and combined across channels. Note that the RGB images are used as DNN input. Each color channel captures the same spatial information of objects, while channels are different in appearances due to  their difference in electromagnetic frequencies. DNN performs the isometric convolution independently in each color channel before they are combined to across channels. Similar to RGB images, CSI data captures the same spatial information of objects in each CSI channel. Different channels contain different electromagnetic responses due to difference signal frequencies of subcarriers. Following the same method used in image-based DNN approaches, we process CSI data by putting CSI of subcarriers as the channels of input tensor. 

Second, we enrich the within-channel feature through multi-stage expansion using a generation network. The input of each subcarrier channel is only $1\times 1$, so the 2D convolution of standard DNN for classification and regression tasks is impossible. In order to mine isometric spatial information embedded in CSI channels, a generation network is used to expand the CSI channel into 2D feature maps.  \\



(2) Incomplete description of how CSI data is mapped to the input layer.

\blue{Response:} We add more description of mapping CSI data to the input layer in \Sec{input}. Besides, \Table{shared} and \Figure{net_flow} are also used to show the CSI data mapping process.\\



(3) Results lack sufficient description and detail

\blue{Response:} In the result section, we add more description about features used in SVM and Naive Bayes in \Sec{overall}. Meanwhile, the setting comparison between our work and prior work is added in \Sec{overall}. More explanation on biometric estimation is added in \Sec{bio_result}. An analysis of why CSI-Net achieves 100\% accuracy is added in \Sec{sign_result}. Comparison between sign recognition and falling detection is added in \Sec{falling_result}. Besides, we compare 9 different backbone networks in \Sec{ablation}. In addition, we add \Sec{v15} to test three different methods of reshaping the input CSI sample~($1\times 1$) to image-like tensor ($224 \times 224$). At last, we give some explanation about the difference between jointly training and separately training in \Sec{jointly}\\






(4) Comparison to alternative (non-adapted DNN) is missing (proof of superiority of the work).

\blue{Response:} We show the results of SVM and Naive Bayes algorithms on our dataset in \Table{accuracy}, which is much worse than CSI-Net. Comparison with prior work~(non-adapted DNN) is also shown in \Table{accuracy}. In \Sec{overall}, we give more explanation on comparing our work with prior non-adapted DNN work.\\


\blue{\textit{Please see our responses for other comments in \Sec{other}.}}\\






==> tex/r3_full.tex <==
\noindent\textbf{From reviewer 3}

(1) It is not clear and no evidence is provided
that this is a reasonable choice given that it draws apart neighboring channels through the row-break in the 2D matrices. Unlike in images, for which this design was proposed, the neighborhood relation is therefore not preserved/modeled by the 2D matrices. In addition, the authors do not explain how the remaining samples (e.g. from channels 29, 30 in the case of 2x2 2D matrices); channels 28,29,30 (3x3 matrices); channels 17-30 (4x4 matrices)) are mapped onto the input layers of the neural network. Are these samples discarded? Other than this, there is input-mapping, the DNN is not adapted and it is not clear why this particular mapping is specifically tailored for using CSI data and also why the 2D matrix structure employed in image recognition should be retained for CSI data. It does not respect any specific property of the CSI input such as correlation in neighboring channels. 


\blue{Response:} This may be an unclarity on our manuscript. In our experiments, we always set the channel size of input 30 and never change it. Our proposal is to adjust the $width$ and $height$ of input according to the length of an 
%activity lasting. 
activities' duration. 
In our experiment, we test stationary pose. It is nature that every single-time-point sample can be used to classify an activity. Therefore, the $width$ and $height$ is always $1\times1$. However, if an activity lasts longer and needs more samples to represent, we could reshape them to other shapes, such as $3\times3$, $4 \times 4$, \etc. 
To avoid such misunderstanding, we have removed related content and figure. \\




(2) In particular, I am missing a proof that the applied mapping is actually better than previous approaches in the literature utilizing DNNs with CSI input. For instance, consider 
http://rfpose.csail.mit.edu/. I suggest that the authors employ 1-2 algorithms from the literature to verify the quality and superiority of their approach.


\blue{Response:} We thank the valuable comment. Following your suggestion, we add some related works in \Sec{prior_deep} to prove that the deep learning could be adapted for processing CSI data. Comparing to these works, our contribution is to bring modern CNN into CSI sensing tasks. However, we are not able to employ the algorithms in \href{ http://rfpose.csail.mit.edu/}{ http://rfpose.csail.mit.edu/} 
. The reason is they use FMCW radars, which are not adopted in our work. In fact, their input is not CSI, but a 2D-depth map received from the radar, which can be found at their prior work, \href{ http://rfcapture.csail.mit.edu/}{http://rfcapture.csail.mit.edu/}.\\


(3) For instance, please define CSI in your case? Do we talk about complex-valued I/Q samples? Or, do the authors apply some pre-processing and is it real numbers representing either signal strength or phase of the signal or both?

\blue{Response:} Yes, we are talking about complex-valued I/Q samples. But due to the phase unsuitability of Intel 5300 NICs, we just use the \textit{absolute value} of CSI. We thank the reminder, and have made it more clear in \Sec{input}.\\


(4) Then, why do the authors chose 8 convolutional layers with 7x4x4 and 1x3x3? How is this then mapped to the 30x224x224 tensor? 

\blue{Response:} Generally, the transposed convolutional layer can \textit{double} the $height$ and $width$ of tensors. Taking 224 for example, it should undergo as 224, 112, 56, 28, 14, 7,\blue{...}, 4, 2, 1. We choose 4x4 because our idea is derived from DC-GAN,~\href{https://arxiv.org/pdf/1511.06434.pdf}{https://arxiv.org/pdf/1511.06434.pdf} , which adopts the 4x4 setting.  Meanwhile, there is a gap from 4 to 7. We use a 3x3 kernel to bridge this gap. In the revised manuscript, we have added more details in \Sec{generation}. In the Appendix, we use \Table{shared} and \Figure{net_flow} to show the whole tensor mapping processing with detailed parameters.\\

 

(5) Also, it appears that the authors attempt to classify activities that develop over time (falling) from single-time-point samples over 30 frequencies. This needs further elaboration and motivation. Given the noise in the input, how can such activity be classified from a time-point slice over 30 frequencies?

\blue{Response:}~Yes, we are developing over time (falling) from single-time-point samples over 30 frequencies. We must do this because deep learning usually requires very large datasets. It is not easy for us to ask 30 subjects doing the activity for many times, such as thousands of hundreds of times. In the revised version, we explained this in \Sec{collection}.

To enable classifying the activity merely from a time-point slice, we made comprehensive efforts. First, we applied layered filter to denoise. Second, our input is not the original one-time point but the average of 10-time points, depicted in \Sec{dataset} (Local Temporal Average). At last, we use a data augmentation technology to increase the diversity of training datasets, which makes CSI-Net more robust to noise. In the revised manuscript, we explain the data augmentation algorithm with more descriptions in \Sec{dataset} (Augmenting Training Dataset).\\


(6) In figure 6, why is the training data less stable than the testing data?

\blue{Response:} In \Figure{filter}, we show part of the 15th subcarrier series recorded when the 5th subject is standing at a position. Although the subject is asked to keep still, the environment noise, his/her breathing and heart-beating may cause CSI varying. Besides, it is not easy for him/her to stand for 100 seconds without any movements, so his/her small movements may also result in CSI varying. We make an in-depth discussion about this in Section \Sec{dataset}. Because of these factors, we cannot tell the reason why the training data is less stable than the testing data in this figure. Our data was collected in a controllable and unchanged environment. We add more description in subsection \Sec{collection} as well as \Figure{layout} to show our data collection process.\\  


(7) Where did the ground-truth on the subject's bone-rate come from and did the results match the ground truth? 

\blue{Response:} It is from a Mi\textregistered ~
 body composition scale. \href{https://www.mi.com/us/mi-body-composition-scale/}{https://www.mi.com/us/mi-body-composition-scale/}. In \Sec{collection}, the first line of the Biometrics Estimation part reports this. This is a feasible way for us to get the bone-rate. \\


(8) It is very strange to me that 1) 9/10 signs achieved 100\% (!) accuracy and a single one received much lower accuracy of <95\%. In particular, the explanation of the authors that the symbol 1 is close to 8 is not correct given the gestures
given in figure 5. 8 is much closer to 7 or to 4 and 1 closer to 2 from the images. Can you verify this with a second experiment? 

\blue{Response:} Many thanks for the valuable comment. We have made several other experiments, and found that our previous explanation is not correct. We confess that it is not easy to understand what deep learning have done on the CSI input. We thank the reminder and omit this explanation to avoid misleading. \\

(9) This also made me think about how the experiment was conducted. Is it e.g. possible that not the gesture but the distance of the hand to the receive node impacted the classification? In addition, was the sampling repeated multiple times and with multiple subjects so that exact gesture, hand position and hand size differed? Or, is it such that a single subject held the hand in the LoS between transmitter and receiver for some while and all these samples have been used for the training and testing (This is my guess given the
results).

\blue{Response:} We conducted the experiment with high constraint on the involved subjects. In the revised version, we discuss the constraint in \Sec{collection}~(Sign Recognition). According to our experiment and discussion, we think it is the gesture that impacts the classification. 

``A single subject held the hand in the LoS between transmitter and receiver'' is correct, and we have shown this in the \Table{deployment}~(\# of subjects). Besides, we add \Figure{layout} to confirm this. However, the ``all these samples have been used for the training and testing'' is an unclarity. In all tasks, we use the first 4/5 data for training, and  the remaining 1/5 for testing. We show in \Figure{filter}~(bottom) and describe in its caption. To avoid this misunderstanding, we emphasize the way of splitting training/testing dataset in \Sec{dataset}. 

We also add two paragraphs to explain the reason why CSI-Net can achieve high accuracy for our dataset in \Sec{sign_result} and \Sec{falling_result}. \\


(10) How single-sample CSI data over 30 frequency bands is able to distinguish those gestures. An intuitive explanation would help greatly. Similarly, for the falling detection, I am lost without a better description of the experiment. In particular, please elaborate how slicing out a single time-point sample from the data can be decisive in detecting that activity. Since you are looking not at a time-window and hence can not obtain any information on
e.g. variance, I am completely lost. In particular, please also describe how the activities were labeled. E.g. when does 'falling' start? There are so huge number of time-points in a single falling event and CSI profile from time-point slices should look rather random dependent on how the person falls and also dependent on the persons body mass and size. Detailed information on the subjects is missing too.

\blue{Response:} Many thanks for the comment. We rewrite \Sec{model}. In the revised version, we theoretically elaborate why human presence can cause CSI varying. For the falling detection, we add more description on the experiment \Sec{collection}~(Falling Detection) and a layout figure~(\Figure{layout}). 

Actually, we did not detect an activity in the entire duration.
We are to detect the pose corresponding to an activity. Taking the falling detection for example, subjects are asked to lay on a camp bed, as shown in \Figure{layout}. CSI samples recorded in the whole duration are labeled as ``fallen''. 
Detailed explanation can be referred to the Response to (5). In the previous version, we mentioned this in \Sec{prior_body}~(the last paragraph) and \Sec{prior_activity} (the last paragraph). In the revised version, we emphasize this in \Sec{bio} and \Sec{collection}.\\


(11) For the human identification and Biometrics estimation, I wondered why the `jointly trained performance' actually exceeded the separately trained performance. Considering more classes achieves a better performance if I got this right. Please elaborate on this as it is counter-intuitive.

\blue{Response:} This is because one's identity and biometrics are highly correlated. If the biometrics are estimated correctly, CSI-Net is prone to correctly identifying users. And if the human identification is correct, the biometrics is prone to be estimated rightly. In summary, if we train them jointly, CSI-Net is prone to converge to a state where both tasks achieve a good performance. A more detailed explanation for this concern is added in \Sec{jointly}.\\


(12) In addition, please consider to use the same metric in the table to avoid confusion (e.g. add accuracy information to the Biometrics column and add error information to the identification column).

\blue{Response:} Many thanks for the valuable suggestion. It is hard to find a proper way to use the same metric. This is because biometrics estimation is a regression problem but the other three tasks are classification problems. Taking the body fat rate for example, the value of body fat is a \textit{real} number. To evaluate the performance, we compute the difference between the ground-truth and the estimation value, which results in the metric of $error$. However, it is still difficult to define how accurate the estimation of biometrics is.\\



(13) Please detail how much training and input data was required to achieve your results.

\blue{Response:} We detail the dataset size in \Table{datasize} and add description in \Sec{dataset}~(last paragraph). \\


(14) Section 2 is missing a background section on DNNs for (CSI-based) activity recognition.

\blue{Response:} Following your suggestion, we add \Sec{prior_deep} to show some prior works that apply NNs for CSI data. Existing works only used SHALLOW networks (less than 5 layers), and mainly focused on indoor localization. To our knowledge, there is no existing work that uses DEEP neural network for activity recognition from CSI data.\\


(15) The task stage is not scalable for the identification task: if a 31st subject were added, the complete network has to be rebuild and retrained. Please discuss this and also discuss possible more scalable constructs. 

\blue{Response:} Thanks for addressing the scalability problem. The common practice to solve identification task is to solve as a classification problem. This means predefined and fixed number of classes (30 classes in our experiments). In order to add a 31st identity as a new class, the original 30-class classifiers need to be re-trained for 31 classes. To make the identification task scalable, one can use an identity validation approach. This approach takes two inputs, one gallery sample and one probe sample, and output one scalar indicator if these two samples belong to the same person or not the same person. 

Both approaches have their advantages and drawbacks. The Classification approach is less scalable, but doesn't need to save gallery samples used in training.  The validation approach is scalable, but need to save gallery samples. \\

% To date, in the work of applying CNNs for classification problem, the last layer is fully-connected layer with cross entropy loss, which means the number of cells has to be equal to the number of classes. In fact, in other classification algorithms, such as SVM, logistic regression and decision tree, if a new class was added, the model also has to be retrained. We think this is not a general limitation. 

% We set a variable~(num\_class) to represent the number of classes. Rebuilding CSI-Net is to change the variable according to the number of classes. Besides, retraining CSI-Net may be accelerated by loading a pre-trained model excluding the parameters of the last fully-connected layer, then training it from this pre-trained model.

% Although we cannot avoid the retraining, we have an idea of not rebuilding CSI-Net. The idea is to use regression loss, such as L1, L2 and MSE, to replace the classification loss, cross entropy loss. For example, if we have 3 classes, we annotate them with label of  1/3, 2/3 and 3/3. We can build a DNN that outputs one continuous number and compute the distance between the output and the label. The prediction is the one with the smallest distance. In generic situation, if we have $n$ classes, the annotations can be 1/n, 2/n,..., n/n. The classification strategy is the same as above. Because this idea is counter-intuitive, we do not add it in the discussion section to avoid misleading.\\


(16) To our knowledge this is the first attempt to open the black-box of DNNs on CSI data" 1) this is repeated 1:1 in section 6 and can be omitted therefore once; 2) This assertion is wrong (see the papers mentioned above and, in particular, there is a lot of work on applying DNNs on CSI data for localization) -> please omit the assertion.

\blue{Response:} We omit this assertion in \Sec{evaluation}, meanwhile, we changes the assertion in \Sec{introduction} to a more precise one, ``To our knowledge, this is the first attempt to visualize and analyze the process of DNNs on CSI data''.\\


(17) Biometrics Estimation? should it actually be `Physiological Estimation'?

\blue{Response:} Many thanks for your advice. In the context of our draft, the meaning of `bio-metric-s' is threefold: `bio-' means the human body, `metric' means the fat/muscle/water/bone rate, and `-s' represents the plural of 4 rates. We notice that `biometircs' mainly stands for a college subject, \ie, `the analysis of biological data using mathematical and statistical methods', which does not match our expectation. We have searched these two phases in Google and Google Scholar with quotation marks. Both are widely used, although from the result we find that the number of records of `physiological estimation' is more than that of `biometrics estimation'. Considering the reading coherence, we suggest to continuously use `biometircs estimation'.\\  



(18) Falling detection is only a 2 class problem. Still the performance is much worse compared to e.g. the 10-class problem of detecting finger gestures. Please explain why it is much more difficult to detect a falling subject (whole subject) with the system, compared to changed finger gestures.

\blue{Response:} In the revised version, we add an explanation of this question in \Sec{falling_result}. \\ 







==> tex/r4.tex <==
\noindent \textbf{From reviewer 4}

(1) Empirically show and describe (at least intuitively) that indeed WiFi signals reflecting from one human can contain so much fine grained information about the insides of a human body that one can estimate all these aspects.

% \blue{Response:} We write \Sec{bio} to give an intuition that WiFi signals reflected from one human are embedded with fine grained information of human body. In addition, we rewrite \Sec{model} to theoretically explain that WiFi signals reflecting from one human are embedded with fine grained information of human body.\\
\blue{Response:} We write \Sec{bio} to give an intuition that WiFi signals reflecting from one human are embedded with fine grained information of human body. In addition, we rewrite \Sec{model} to theoretically elaborate this intuition.\\

% we investigated the market and knew that most existing commercial body-composition-scales utilize the electrical resistance of skin, muscle, water, etc., in human body to estimate the body composition.
% Some prior works also show that electromagnetic wave would be influenced if traveling through the human body. 
% In paper xx, the authors modeled the interaction between EM wave and human body. 
% In paper xx, the authors tested the influence of human body components, such as fat, muscle and bone, via EM waves with 900MHz-20GHz.

% We believe body composition can also be estimated through its dielectric constant which is encoded in the CSI data of WiFi. Besides, CNN is a powerful and universal function approximator. It helps us to estimate this fine-grained information.



(2) Provide more detailed description of data collection process and evaluation. Furthermore, collect data such that it incorporates the impact of various real world aspects such as changes to the environment, changes to the positions and orientations of user, impact of the presence of other users in the environment \etc. Include layout figure.

\blue{Response:} We add the site snapshots and layout figures of all 4 sensing tasks in \Figure{layout}. We give more detailed description of data collection in \Sec{collection}, which is to show that our data collection is done within an environment that is controllably unchanged. The changes include 
%ing the changes to the environment, changes 
the ones of the positions and orientations of users, impact of the presence of other users in the environment, and the like. We add more description about splitting training/testing dataset in \Sec{dataset}. 

In the evaluation section, we add more description about features used in SVM and Naive Bayes in \Sec{overall}. Meanwhile, the setting comparison between our work and prior work is added in \Sec{overall}. More explanation on biometric estimation is added in \Sec{bio_result}. An analysis of why CSI-Net achieves 100\% accuracy is added in \Sec{sign_result}. Comparison between sign recognition and falling detection is added in \Sec{falling_result}. Besides, we compare 9 different backbone networks in \Sec{ablation}. At last, we add \Sec{v15} to test three different methods to reshape the input CSI sample~($1\times 1$) to image-like tensor ($224 \times 224$).\\



(3) Demonstrate that the accuracies shown in the results are not due to distinct environmental characteristics at the time of data collection.

\blue{Response:} We detail our data collection part in \Sec{collection}, where we demonstrate that the accuracies we shown in the results are not because of distinct environmental characteristics.\\

(4) Provide comparison with accuracies reported in prior work in comparable scenarios.

\blue{Response:} In \Sec{overall}, we compared our work with several closely-related prior work. Although it is very difficult to re-produce every prior scenarios, in our experiments, we have tried our best to follow the prior experimental settings, such as selection of hand sign, distance/height of Tx/Rx and subject's sitting poses. (please see details in \Sec{collection}). To our knowledge, none of existing work demonstrates the capability as CSI-Net, which serves as a generic framework and achieve good performance in all compared WiFi sensing tasks.  

Moreover, CSI-Net is a flexible deep neural network approach. Given more data from different scenarios, and by choosing heavier backbone networks, CSI-Net can be powerful enough to solve WiFi sensing tasks under various scenarios. \\

\blue{\textit{Please see our responses for other comments in \Sec{other}.}}\\




==> tex/r4_full.tex <==
\noindent\textbf{From reviewer 4}

(1) On Page 2, the authors state that "Each subcarrier has a distinctive frequency and contains independent information of the subcarrier’s interaction with human bodies." This is not really correct. The information about human movements across different subcarriers is highly correlated. This correlation is actually the basis of the noise removal techniques that prior works on WiFi based human activity/gesture recognition systems have proposed.

\blue{Response:} This may be an unclarity, we using the word of \textit{independent} here is to say one subcarrier would not be affected by other subcarriers during it propagating. To avoid this misunderstanding, we omit this word in the revised manuscript.\\


(2) What is the motivation behind showing the figure on the right in Figure 2. Do the authors intend to show some kind of signal diffraction as it propagates through human body? What is the basis behind such propagation. Furthermore, how such propagation leads to the identification of human and his/her biometrics? 

What is the motivation behind including Section 3: Wireless Signal Model? The content described in this section is common knowledge and has not be referred to or used in the rest of the paper. Similarly, Table 1 provides no information that is relevant to the the technical content of the paper.

\blue{Response:} We thank the valuable comment. In the original version, this was expected to show an intuition that human presence can cause CSI variances. In the revised version, we rewrite \Sec{model}. The new \Sec{model} along with \Sec{bio} show that WiFi signals reflected by human body are embedded with fine-grained human body information, which would make \Figure{body} and \Table{tissue} more relevant to the manuscript. \\


(3) As per my understanding, the proposed system just learnt the characteristics of the environment at the time the authors collected data and the system overfitted on it to get high accuracy. The authors need to provide more information about their data collection and evaluation processes. What scenarios were the data collected in. How were the user orientations and positions changed when collecting data. Was the surrounding environment static? The authors should include a layout figure of the environment.


Regarding the part about sign language detection, again, more details are needed about how the samples are collected. Does the system recognize the motion of making a certain hand signs or recognizes the stationary pose of the hand? 

\blue{Response:} We thank the suggestion, we add more data collection details in \Sec{collection}. Besides, we add a data collection site figure and a layout figure~(\Figure{layout}) for every task.\\


(4) Algorithm 1 is not clear. The authors should provide more description in the text to explain it.

\blue{Response:} Many thanks for the comments. In the revised version, we provide more description in the \Sec{dataset}~(Augmenting training dataset) to explain \Algorithm{augmentation}.\\


(5) Regarding the data collection, the authors should explain more as to how the training samples were selected, how many samples were selected for training and how many for testing etc.

\blue{Response:} We thank the valuable advice. In the revised version, we detail training sample selection method in \Sec{dataset}~(first paragraph). We also report the number of training/testing samples in \Table{datasize} and describe it in the \Sec{dataset}~(last paragraph). \\



(6) For SVM and Naive bayes in Table 7, what features were used? 

\blue{Response:} It is the same as the features for CSI-Net. Following your suggestion, we emphasize this in \Sec{overall}~(first paragraph). \\


% (7) On three out of the four problems that the authors have evaluated on, i.e., human identification (e.g. [1], although it requires the user to walk), sign recognition (e.g. [2]), fall detection (e.g., [3]), researchers have previously proposed solutions and evaluated them in quite diverse settings. The authors should evaluate their scheme in similar settings and compare their results with these.

% \textbf{Response:} We thank the suggestion, we add more description on data collection and display our experiment is in a similar setting as comparing with prior work in data collection part, 5.1.2.







==> tex/r5.tex <==
\noindent\textbf{From reviewer 5}

(1) More details about the sample data collection process.

\blue{Response:} We add the site snapshots and layout figures of all 4 sensing tasks in \Figure{layout}. We give more detailed description of data collection in \Sec{collection}, which shows that our data collection is done within 
an environment that is controllably unchanged. The changes include 
the ones of the positions and orientations of users, impact of the presence of other users in the environment, and the like.
%controllable environment unchanged including the changes to the environment, changes to the positions and orientations of user, impact of the presence of other users in the environment \etc. 
We add more description about splitting training/testing dataset in \Sec{dataset}. \\


(2) Explanation of WiFi signal variation in relation with presence of human body.

\blue{Response:} We write \Sec{bio} to give an intuition that WiFi signals reflecting from one human are embedded with fine grained information of human body. In addition, we rewrite \Sec{model} to theoretically elaborate this intuition.
%that WiFi signals reflecting from one human are embedded with fine grained information of human body.
\\



(3) Amount of training data samples and testing data part during the experiment. How the training samples were selected, how many samples were selected. Should clearly explain about cross-validation technique.

\blue{Response:} The amounts of training samples and testing data are listed in \Table{datasize}. Meanwhile, we add more description in the last paragraph of \Sec{dataset} to emphasize it. We make the way to select training data clear by adding the 1st and 2nd paragraphs of \Sec{dataset}. 

In fact, we did not apply cross-validation techniques. In all tasks, we selected the first 4/5 samples for training and the last 1/5 samples for testing. We took this splitting strategy to simulate the practical scenarios, where one first collects data and trains a network, then tests incoming data. As shown in \Table{accuracy}, \Table{bio} and \Figure{bio},  CSI-Net works well in all tasks, although CSI sequences have noises as plotted in \Figure{filter}.\\


\blue{\textit{Please see our responses for other comments in \Sec{other}.}}\\


==> tex/r5_full.tex <==
\noindent\textbf{From reviewer 5}

(1) The issue tackled by the paper is interesting and relevant in the field; author claim about the work as a first work to estimate human biometrics using WiFi signal but related previous work should address properly with references.

\blue{Response:} We thank the valuable suggestion. In the revised version, related previous approaches about biometrics estimation are addressed in \Sec{bio}.\\


(2) In section 4.3, feature learning stage which is core component of CSI-Net should be written more clearly. Why you compare ResNet-34 and 56. Propose approach and discussion part is also need to elaborate with the originality of this work.

\blue{Response:} Following your suggestion, we rewrite the \Sec{feature_learning}. In the new \Sec{feature_learning}, we explain why we choose ResNet-18. In addition, we add \Sec{ablation}, \Table{backbone} and \Table{modelsize}, to explain the reason of using experimental results. There, we compare 9 different networks and conclude that ResNet-18 is most suitable for our dataset.


